Self-Supervised 3D Face Reconstruction via Conditional Estimation

We present a conditional estimation (CEST) framework to learn 3D facial parameters from 2D single-view images by self-supervised training from videos. CEST is based on the process of analysis by synthesis, where the 3D facial parameters (shape, reflectance, viewpoint, and illumination) are estimated from the face image, and then recombined to reconstruct the 2D face image. In order to learn semantically meaningful 3D facial parameters without explicit access to their labels, CEST couples the estimation of different 3D facial parameters by taking their statistical dependency into account. Specifically, the estimation of any 3D facial parameter is not only conditioned on the given image, but also on the facial parameters that have already been derived. Moreover, the reflectance symmetry and consistency among the video frames are adopted to improve the disentanglement of facial parameters. Together with a novel strategy for incorporating the reflectance symmetry and consistency, CEST can be efficiently trained with in-the-wild video clips. Both qualitative and quantitative experiments demonstrate the effectiveness of CEST.

==> framework.tex <==
Common self-supervised approaches to 3D face reconstruction estimate the facial parameters in an analysis-by-synthesis manner. Specifically, the learning process is formulated as training an autoencoder that decomposes the face image into shape, reflectance, viewpoint and illumination, and subsequently recombines these model parameters to reconstruct the original image. The estimation problem can be formulated as $P(\hat{\bm{I}}|\bm{I})=P(\mathcal{R}(\bm{S}, \bm{R}, \bm{v}, \bm{\ell})|\bm{I})$, where $\bm{I}$, $\hat{\bm{I}}$, $\bm{v}$, and $\bm{\ell}$ are the given image, reconstructed image, viewpoint, and illumination parameters, respectively. $P(\hat{\bm{I}}|\bm{I})$ is the posterior probability of $\hat{\bm{I}}$ given $\bm{I}$,  and $\mathcal{R}$ is a differentiable renderer. Since the renderer $\mathcal{R}$ is a deterministic model with no learnable parameter, we have $P(\mathcal{R}(\bm{S}, \bm{R}, \bm{v}, \bm{\ell})|\bm{I})=P(\bm{S}, \bm{R}, \bm{v}, \bm{\ell}|\bm{I})$.

To obtain the facial parameters (shape, reflectance, viewpoint and illumination), previous approaches \cite{tran2018nonlinear,tewari2017mofa,zhou2019dense} construct a shared (or separated) module(s) to perform the prediction independently. Without the loss of generality, we represent the independent predictions with separated modules as $P(\bm{S}, \bm{R}, \bm{v}, \bm{\ell}|\bm{I})=P(\bm{S}|\bm{I})P(\bm{R}|\bm{I})P(\bm{v}|\bm{I})P(\bm{\ell}|\bm{I})$\footnote{For shared modules, the independent predictions can formulated as $P(\bm{S}|\bm{z})P(\bm{R}|\bm{z})P(\bm{v}|\bm{z})P(\bm{\ell}|\bm{z})P(\bm{z}|\bm{I})$, where $\bm{z}$ is the shared latent representation.}. We note that this formulation implicitly makes a conditional independence assumption: the facial parameters ($\bm{S}, \bm{R}, \bm{v}, \bm{\ell}$) are independently predicted given the image $\bm{I}$. However, this assumption is not necessarily true. For example, the pixel values in an image are the joint consequence of the shape (normal), reflectance, and illumination. These facial parameters are hence statistically dependent on each other given the image, and the assumption of conditional independence is questionable.

In CEST, we predict the facial parameters {\em sequentially}. As shown in Fig. \ref{fig:cest_framework}, we model the estimations for viewpoint, shape, reflectance, and illumination as  $P(\bm{v}|\bm{I})$, $P(\bm{S}|\bm{I}, \bm{v})$, $P(\bm{R}|\bm{I}, \bm{v}, \bm{S})$, and $P(\bm{\ell}|\bm{I}, \bm{v}, \bm{S}, \bm{R})$, respectively. As can be seen, the prediction of each facial parameter is conditioned on the original image and the facial parameters that have been derived. As a result, the coupling between the facial parameters occurs not only through the reconstruction, but also during the inference, providing additional mutual constraints for each other. Most importantly, the estimation problem in CEST is formulated as $P(\bm{S}, \bm{R}, \bm{v}, \bm{\ell}|\bm{I}) = P(\bm{v}|\bm{I})P(\bm{S}|\bm{I}, \bm{v})P(\bm{R}|\bm{I}, \bm{v}, \bm{S})P(\bm{\ell}|\bm{I}, \bm{v}, \bm{S}, \bm{R})$ , which is the original formulation $P(\bm{v}, \bm{S}, \bm{R}, \bm{\ell}|\bm{I})$ and no conditional independence is assumed. 
%\wy{We should explicitly emphasize our method does not require conditional independence.}

During inference, the expert-designed rendering module is not required. CEST is able to predict the 3D facial parameters, namely shape, reflectance, and illuminance, from a single image.


